Cem Mil Podcasts: A Spoken Portuguese Document Corpus For Multi-modal, Multi-lingual and Multi-Dialect Information Access Research

In this paper we describe the Portuguese-language podcast dataset we have released for academic research purposes. We give an overview of how the data was sampled, descriptive statistics over the collection, as well as information about the distribution over Brazilian and Portuguese dialects. We give results from experiments on multi-lingual summarization, showing that summarizing podcast transcripts can be performed well by a system supporting both English and Portuguese. We also show experiments on Portuguese podcast genre classification using text metadata. Combining this collection with previously released English-language collection opens up the potential for multi-modal, multi-lingual and multi-dialect podcast information access research.

==> archive/3_data_overview.tex <==
\section*{Data Overview}
For each episode, we provide the audio file, the transcription of this audio file and the associated metadata. The following metadata is provided:
\begin{itemize}
\item show\_uri: Spotify uri for the show. (e.g. spotify:show:2GfMFAmQseZ1fOtiLQyZ39)
\item show\_name: Name of the show. (e.g. ``Hoje no TecMundo Podcast'')
\item show\_description: Description of the show. (e.g. ``O Hoje no TecMundo é o tradicional programa diário do TecMundo no YouTube...”)
\item publisher: Publisher of the show. (e.g. Hoje no TecMundo - Podcast)
\item language: Language the show is in in BCP 47 format. (e.g. pt-BR)
\item rss\_link: links of show rss feed. (e.g. https://anchor.fm/s/11c4550c/podcast/rss)
\item episode\_uri: Spotify uri for the episode. (e.g. spotify:episode:7otAzBBGK7uwqhxV3kWwLm)
\item episode\_name: Name of the episode. (e.g. "Hoje no TecMundo 17/01/2020 – Preço do Galaxy Fold no Brasil, imagens do Huawei P40 Pro")
\item episode\_description: Description of the episode. (e.g. “No programa de hoje, falamos do preço caríssimo do Galaxy Fold no Brasil, a Google prometendo...”)
\item duration: duration of the episode in minutes. (e.g. 9.113833333333334)
\item show\_filename\_prefix: Filename\_prefix of the show. (e.g. show\_2GfMFAmQseZ1fOtiLQyZ39)
\item episode\_filename\_prefix: Filename\_prefix of the episode. (e.g. 7otAzBBGK7uwqhxV3kWwLm)
\end{itemize}

We also provide the RSS feeds for each podcast show. This is a rich source of metadata which enables a number of different perspectives for a research project.


% Genre distribution
In Table \ref{tab:pt-genre}, we can see the distribution of episodes per genre. The top 5 genres account for 69\% of all episodes. Business, Education, Sports and Comedy are part of the top 5 genres of both the English and Portuguese podcasts dataset.


\begin{table*}[th]
\centering
\begin{tabular}{|r|r|}
\hline
\textbf{Genre}           %& \textbf{Number of Episodes} 
& \textbf{Number of Episodes} \\ 
                         %& \textbf{in English Dataset} 
                         & \textbf{in Portuguese Dataset} \\ \hline
Business                 %&
& 26~915                   \\ \hline
Education                %&                              
& 23~541                   \\ \hline

Sports                   %&                              
                               &13~467                   \\ \hline
Comedy                   %&                              
                               &11~211                   \\ \hline

Arts                     %&                              
                               &9~869                    \\ \hline
TV \& Film               %&                              
                               &5~451                    \\ \hline

Science                  %&                              
                              & 5~379                    \\ \hline
Music                    %&                              
                               & 3~952                    \\ \hline

Technology               %&                              
                               & 3~193                    \\ \hline
Society \& Culture       %&                              
                               & 3~192                    \\ \hline

Kids \& Family           %&                              
                              & 3~036                    \\ \hline
Leisure                  %&                              
                              & 2~756                    \\ \hline

Health \& Fitness        %&                              
                              & 2~337                    \\ \hline
History                  %&                              
                              & 2~254                    \\ \hline

Fiction                  %&                              
                              & 2~024                    \\ \hline
True Crime               %&                              
                              & 1~749                    \\ \hline

News                     %&                              
                              & 1~098                    \\ \hline
Religion \& Spirituality %&                              
                              & 1~037                    \\ \hline

Government               %&                              
                              & 531                     \\ \hline
None                     %&                              
                              & 62                      \\ \hline
\end{tabular}
\caption{Portuguese Podcasts dataset: number of episodes per genre}
\label{tab:pt-genre}
\end{table*}

%\section*{Language Use and Dialect}
%\label{sec:dialect}
%In this Section we drill down into the kinds of language used in the podcasts, as well as the dialect spoken. 

% from older dataset
% [['eu', 0.013155929583958337], ['tu', 3.896129195644128e-05], ['você', 0.004840940525587829], ['cê', 1.2987097318813758e-05], ['ele', 0.008295508412392289], ['ela', 0.0025357307514983865], ['nós', 0.0016720887797972714], ['nóis', 0], ['vós', 1.6233871648517198e-05], ['vóis', 0], ['vocês', 9.74032298911032e-06], ['cês', 0], ['eles', 0.001152604887044721], ['elas', 0.00021428710576042702]]
% 
%\begin{table}[]
%    \centering
%    \begin{tabular}{|l|c|c|} \hline
%    Pronoun (and gloss)    & Prob & odds ratio relative to 'eu' \\ \hline
%    eu  (I)   & 0.131 & 1 \\
%    tu (you - singular, familiar) & 3.896 & 29.7 \\
%    você (you - singular, more formal) & 0.005 & 0.036 \\
%    cê (??) & 1.299 & 9.916 \\
%    ... & & \\
%   \hline
%    \end{tabular}
%    \caption{Distribution over pronouns over the entire Portuguese collection. (Currently computed over 50k episodes, to be recomputed over entire collection}
%    \label{tab:my_label}
%\end{table}
% https://en.wikipedia.org/wiki/Portuguese_personal_pronouns#Basic_forms

\section*{Access to the dataset}


%%% The Portuguese language podcast dataset is available for non-commercial research purposes in the same way and under the same agreement as the English language podcast dataset. The English language podcast dataset has been most notably used in shared tasks on segment retrieval and summarization in TREC 2020 \cite{jones2020trec} and TREC 2021 \cite{karlgren2021trec} but is also currently used for many other research purposes such as document segmentation or dialogue modelling and there are several annotations and enrichments such as a search index, human assessments, and precomputed audio features available for the English language section. We expect that this extension will broaden the scope of research and lower the threshold to apply methods to more than one language. We welcome contributions to further enrich the dataset through annotations of various kinds. 
%%% 
%% To request the dataset, please go to \url{https://podcastsdataset.byspotify.com/} and follow the instructions.

\noindent
\fbox {
    \parbox{0.9\linewidth}{
    {
    \begin{center}
        \large \tt  
        Procedure to access the dataset will be given here at time of publication; anonymised for now. 
        
        It will be available for non-commercial research purposes. 
    \end{center}
    }
    }
    }


==> archive/sections/2_introduction.tex <==
\section*{Portuguese Podcast Dataset for Academic Research}
Podcasts, a new and emergent spoken mass communication medium, come in many formats and levels of formality. Podcasts are typically produced as topically or stylistically consistent \textit{shows} which consist of \textit{episodes}, which are published serially with some regularity over time. Podcast shows can be educational, journalistic, or fictional; formal or informal; conversational or monologues; and vary over type, style, form, and topic. Podcast consumption has been growing rapidly \cite{whitner2020meteoric} and podcasts have in the past years become a topic of interest for research in speech and language technology, linguistics, information access technology, and media studies. Podcasts are available in a wide variety of languages. The Anchor podcast creation app is available in thirty-five languages \cite{anchorUILanguages} with many more podcasters creating podcasts in other languages. %  (give statistics over Spotify?


In order to facilitate academic research on podcasts, Spotify released an English language podcast dataset for research purposes in 2020 \cite{clifton2020hundredthousand}. That dataset has been shared to more than one thousand research groups since it was published. It is orders of magnitude larger than previous transcribed speech datasets, and contains a rich variety of genres, subject matter, speaking styles, and structural formats, departing from other collections of English language data \cite{karlgren2022lexical}. 

However, research on English alone risks results to be overly specific to one language and one cultural arena. To address this source of bias, we have compiled a complementary dataset in Portuguese, of comparable size and breadth. In addition, like the English dataset, it contains metadata that can be used as proxy labels for supervised learning tasks, such as creator descriptions for the summarization task and show publisher for authorship attribution tasks.

The Portuguese language is the sixth most-spoken language in the world, with 250 million native speakers, in many cultural areas, and with 24 million more L2 speakers \cite{portLangWikipedia}.
% possible papers to cite about podcasts in Portuguese, or cite our own data?
% Examining Independent Podcasts in Portuguese iTunes  https://link.springer.com/chapter/10.1007/978-3-030-50732-9_20 
% Audience transformations and new audio experiences: An analysis of the trends and consumption habits of podcasts by Brazilian listeners https://www.researchgate.net/profile/Fabio-Giacomelli-3/publication/351492923_Audience_transformations_and_new_audio_experiences_An_analysis_of_the_trends_and_consumption_habits_of_podcasts_by_Brazilian_listeners/links/609aa1eba6fdccaebd24eb6a/Audience-transformations-and-new-audio-experiences-An-analysis-of-the-trends-and-consumption-habits-of-podcasts-by-Brazilian-listeners.pdf
% This might be a bad one without good source: Invisible audio: an analysis of the podcasts of Portuguese newspapers, https://www.researchgate.net/publication/326235292_Invisible_audio_an_analysis_of_the_podcasts_of_Portuguese_newspapers
Morais et al \cite{morais2021audience} surveyed 566 Brazilian podcast listeners, and found that they listen to podcasts across a range of topic areas, and like information that is complementary to the information found in other media. There have been smaller-scale studies of Portuguese podcasts \cite{antunes2020examining}. % maybe add some more
% Examining Independent Podcasts in Portuguese iTunes  https://link.springer.com/chapter/10.1007/978-3-030-50732-9_20 
We know of no previous large-scale study of Portuguese language podcasts. In order to facilitate research on podcasts in Portuguese, we now release a podcast dataset consisting of 123,054 podcast episodes in Portuguese from 16,131 shows, encompassing more than 76,000 hours of speech audio. This extends the English language podcast dataset with a Portuguese language podcast dataset, effectively more than doubling the collection size.

\section*{Composition and Selection of the Dataset}
The Portuguese language podcast episodes were randomly selected from podcasts that were published between September 9, 2019 and March 31, 2022. 

The process to build the Portuguese language podcast dataset followed the procedure used 
by Spotify %%% remove for camera ready
to build the English language podcast dataset as detailed in the description of that dataset \cite{clifton2020hundredthousand}. The filters used in this process were as follows.

\begin{itemize}
\item The language of the show must be Portuguese (pt-BR or pt-PT)
\item The episode must have more than 50\% of speech over its duration. A proprietary speech detection algorithm was used here. This filters out podcasts which contain mostly music, white noise or ambient sounds, rather than speech. 
%%%  uncomment for camera ready \item The episodes are all Spotify owned-and-operated, for copyright reasons.
\item The episode descriptions must be identified as Portuguese by the langid Python package \cite{lui-baldwin-2012-langid}.
\end{itemize}

All episodes have been transcribed to text with Azure's speech-to-text service\footnote{https://docs.microsoft.com/en-us/azure/cognitive-services/speech-service/index-speech-to-text} which requires a target language and regional variant to be specified. In this dataset this can be either pt-PT (Portuguese from Portugal) or pt-BR (Portuguese from Brazil). We used the following heuristics based on the available episode and show metadata to select the target language:
\begin{enumerate}
\item if the show language is `pt-PT' or `pt-BR', use that as the language for transcription.
\item if the episode language is `pt-PT' or `pt-BR', use that as the language for transcription.
\item if the show's country of origin is `pt' or `br', set the transcription language as `pt-PT' or `pt-BR' accordingly.
\item otherwise, fall back to `pt-BR' because the number of podcast producers in Brazil is larger.
\end{enumerate}


In the end, 114,387 episodes were transcribed using pt-BR and 8667 were transcribed using pt-PT as a target. Examples of each are shown in Figure~\ref{fig:transcript}. Some manual inspection reveals that some classification errors between pt-PT and pt-BR remain: words such as ``\textit{legal}'', Brazilian for ``cool'' or the Brazilian-only pronoun ``cê'' appear in the pt-PT set.
% We drill down further into the languages and dialects spoken in the podcasts in the section on Language Use and Dialect.
% \ref{sec:dialect}.


\begin{figure}
\centering
\begin{tabular}{|lp{0.8\textwidth}|}
\hline
pt-PT & {\small
\textit{Olá \textbf{és} curioso sobre o que se passa no mundo, gosta de saber o que afetou diversosecossistemas e como podes ajudá-los. E esta ao \textbf{sítio} certo, não podcast e como escola São Pedro do Sul, \textbf{podes} encontrar informação sobre o ambiente, novidades relacionadas com o nosso planeta e muitas curiosidades, incluindo as diversas medidas que podes aplicar para ajudares a proteger a natureza. \textbf{Serás} capaz de aprofundar os teus conhecimentos sobre diversos temas, desde alterações climáticas até ao ruído. A \textbf{equipa} de 2 ou 3 vezes por mês que vai contar tudo é composta pelo Miguel Almeida, Rodrigo Cardoso. Tiago Rocha e Filipe Correia. Para não perder nada, subscreve. Já o nosso podcast na tua plataforma preferida e não te esqueças após cada episódio, Podes sempre visitar o nosso website para saberes mais.} } \\
 \hline
pt-BR &
{\small
\textit{ Olá \textbf{você} que é nosso ouvinte do podcast de arte saúde o fiba hoje estaremos nossa segunda entrevista e contaremos com a presença de uma convidada mais do que especial? Ela estéfane psicóloga e arte terapeuta. Oi eu sou estefani eu sou psicóloga formada pela universidade de Passo Fundo com especialização em arteterapia também pela universidade de Passo Fundo e recentemente eu encontrei uma ponte entre a psicologia e a arte terapia através de uma especialização em psicologia clínica e um. Indo pela fam acne Porto Alegre eu \textbf{tô} muito feliz com o convite da área de saúde para falar um pouquinho sobre esse assunto que deixa o meu coração tão quentinho que é arte terapia é sempre % muito prazeroso poder falar sobre esse tema eu estou muito feliz também com essa conexão que a internet possibilitou nessa conexão da Bahia com o Rio Grande do Sul. Muito legal estéfane um currículo assim sensacional e eu fico muito feliz também com essa possibilidade de conectar ideias né de conectar saberes que a internet nos proporciona
…}}
 \\
 \hline
\end{tabular}
    \caption{Example transcripts for the two target varieties of Portuguese. The pt-PT example was extracted from the show ``EESPS: Podcast sobre o ambiente''. The pt-BR was extracted from the show ``Arte e Saúde - UFBA''}
    \label{fig:transcript}
\end{figure}

\section*{Descriptive Statistics}

In Table \ref{tab:pt-general-stats}, we give some descriptive statistics for the Portuguese dataset and compare them to the previously released English dataset. % Are there any interesting differences?


%%% do we want this bit The way podcasts are used differ from some other text and speech data  \cite{jonesEA2021currentchallenges,carterette2021podcast}



\begin{table*}[htbp]
\centering
\begin{tabular}{|r|r|r|}
\hline
     & English & Portuguese  \\
\hline
Number of episodes     & 105 360 & 123 054\\
    Number of shows     &      18 376  &  16 131 \\
\hline
    Average episode duration (minutes) & 33.8 & 37.3 \\
- 25\% & 13.6 & 10.9  \\ 
- 50\% & 31.6 & 31.2   \\ 
- 75\% & 50.4 & 55.0   \\ 
- max   & 305 & 695  \\ 
\hline
    Average number of words (from transcript)  &  5 700 &  9 539  \\
%- 25\% & & 2 203                 &   \\ 
%- 50\% & & 6 746                 &   \\ 
%- 75\% & & 13 693                &   \\ 
%- max                        & & 205 163   &  \\ 

\hline
\end{tabular}
\caption{Descriptive statistics for the Portuguese Language Podcast Dataset, with corresponding data for the previously released English Language Podcast Dataset given as comparison.}
\label{tab:pt-general-stats}
\end{table*}




==> archive/sections/3_data_overview.tex <==
\section*{Data Overview}
For each episode, we provide the audio file, the transcription of this audio file and the associated metadata. The following metadata is provided:
\begin{itemize}
\item show\_uri: Spotify uri for the show. (e.g. spotify:show:2GfMFAmQseZ1fOtiLQyZ39)
\item show\_name: Name of the show. (e.g. ``Hoje no TecMundo Podcast'')
\item show\_description: Description of the show. (e.g. ``O Hoje no TecMundo é o tradicional programa diário do TecMundo no YouTube...”)
\item publisher: Publisher of the show. (e.g. Hoje no TecMundo - Podcast)
\item language: Language the show is in in BCP 47 format. (e.g. pt-BR)
\item rss\_link: links of show rss feed. (e.g. https://anchor.fm/s/11c4550c/podcast/rss)
\item episode\_uri: Spotify uri for the episode. (e.g. spotify:episode:7otAzBBGK7uwqhxV3kWwLm)
\item episode\_name: Name of the episode. (e.g. "Hoje no TecMundo 17/01/2020 – Preço do Galaxy Fold no Brasil, imagens do Huawei P40 Pro")
\item episode\_description: Description of the episode. (e.g. “No programa de hoje, falamos do preço caríssimo do Galaxy Fold no Brasil, a Google prometendo...”)
\item duration: duration of the episode in minutes. (e.g. 9.113833333333334)
\item show\_filename\_prefix: Filename\_prefix of the show. (e.g. show\_2GfMFAmQseZ1fOtiLQyZ39)
\item episode\_filename\_prefix: Filename\_prefix of the episode. (e.g. 7otAzBBGK7uwqhxV3kWwLm)
\end{itemize}

We also provide the RSS feeds for each podcast show. This is a rich source of metadata which enables a number of different perspectives for a research project.


% Genre distribution
In Table \ref{tab:pt-genre}, we can see the distribution of episodes per genre. The top 5 genres account for 69\% of all episodes. Business, Education, Sports and Comedy are part of the top 5 genres of both the English and Portuguese podcasts dataset.


\begin{table*}[th]
\centering
\begin{tabular}{|r|r|}
\hline
\textbf{Genre}           %& \textbf{Number of Episodes} 
& \textbf{Number of Episodes} \\ 
                         %& \textbf{in English Dataset} 
                         & \textbf{in Portuguese Dataset} \\ \hline
Business                 %&
& 26~915                   \\ \hline
Education                %&                              
& 23~541                   \\ \hline

Sports                   %&                              
                               &13~467                   \\ \hline
Comedy                   %&                              
                               &11~211                   \\ \hline

Arts                     %&                              
                               &9~869                    \\ \hline
TV \& Film               %&                              
                               &5~451                    \\ \hline

Science                  %&                              
                              & 5~379                    \\ \hline
Music                    %&                              
                               & 3~952                    \\ \hline

Technology               %&                              
                               & 3~193                    \\ \hline
Society \& Culture       %&                              
                               & 3~192                    \\ \hline

Kids \& Family           %&                              
                              & 3~036                    \\ \hline
Leisure                  %&                              
                              & 2~756                    \\ \hline

Health \& Fitness        %&                              
                              & 2~337                    \\ \hline
History                  %&                              
                              & 2~254                    \\ \hline

Fiction                  %&                              
                              & 2~024                    \\ \hline
True Crime               %&                              
                              & 1~749                    \\ \hline

News                     %&                              
                              & 1~098                    \\ \hline
Religion \& Spirituality %&                              
                              & 1~037                    \\ \hline

Government               %&                              
                              & 531                     \\ \hline
None                     %&                              
                              & 62                      \\ \hline
\end{tabular}
\caption{Portuguese Podcasts dataset: number of episodes per genre}
\label{tab:pt-genre}
\end{table*}

%\section*{Language Use and Dialect}
%\label{sec:dialect}
%In this Section we drill down into the kinds of language used in the podcasts, as well as the dialect spoken. 

% from older dataset
% [['eu', 0.013155929583958337], ['tu', 3.896129195644128e-05], ['você', 0.004840940525587829], ['cê', 1.2987097318813758e-05], ['ele', 0.008295508412392289], ['ela', 0.0025357307514983865], ['nós', 0.0016720887797972714], ['nóis', 0], ['vós', 1.6233871648517198e-05], ['vóis', 0], ['vocês', 9.74032298911032e-06], ['cês', 0], ['eles', 0.001152604887044721], ['elas', 0.00021428710576042702]]
% 
%\begin{table}[]
%    \centering
%    \begin{tabular}{|l|c|c|} \hline
%    Pronoun (and gloss)    & Prob & odds ratio relative to 'eu' \\ \hline
%    eu  (I)   & 0.131 & 1 \\
%    tu (you - singular, familiar) & 3.896 & 29.7 \\
%    você (you - singular, more formal) & 0.005 & 0.036 \\
%    cê (??) & 1.299 & 9.916 \\
%    ... & & \\
%   \hline
%    \end{tabular}
%    \caption{Distribution over pronouns over the entire Portuguese collection. (Currently computed over 50k episodes, to be recomputed over entire collection}
%    \label{tab:my_label}
%\end{table}
% https://en.wikipedia.org/wiki/Portuguese_personal_pronouns#Basic_forms

\section*{Access to the dataset}


%%% The Portuguese language podcast dataset is available for non-commercial research purposes in the same way and under the same agreement as the English language podcast dataset. The English language podcast dataset has been most notably used in shared tasks on segment retrieval and summarization in TREC 2020 \cite{jones2020trec} and TREC 2021 \cite{karlgren2021trec} but is also currently used for many other research purposes such as document segmentation or dialogue modelling and there are several annotations and enrichments such as a search index, human assessments, and precomputed audio features available for the English language section. We expect that this extension will broaden the scope of research and lower the threshold to apply methods to more than one language. We welcome contributions to further enrich the dataset through annotations of various kinds. 
%%% 
%% To request the dataset, please go to \url{https://podcastsdataset.byspotify.com/} and follow the instructions.

\noindent
\fbox {
    \parbox{0.9\linewidth}{
    {
    \begin{center}
        \large \tt  
        Procedure to access the dataset will be given here at time of publication; anonymised for now. 
        
        It will be available for non-commercial research purposes. 
    \end{center}
    }
    }
    }


==> archive/sections/4_summarization.tex <==
\section*{Summarization}

Automatic Text Summarization is the task of taking a source document as an input and producing a much shorter version of it while preserving the most important pieces of information. In \cite{clifton2020hundredthousand}, the authors trained a transformer-based model to summarize transcripts of podcast episodes in English. Traditional transformer-based model are usually limited to 512 or 1024 tokens as an input which is very restrictive to transcripts. In Table \ref{tab:pt-general-stats}, we see that transcripts of podcasts in Portuguese have on average 9539 words. In this work, we have experimented not only with traditional transformer-based models but also with Longformer-based\cite{beltagy2020longformer} models with input sizes of 4096 tokens.

\subsection*{Boilerplate annotations in episode descriptions in Portuguese} \label{sec:boilerplate}
Episode descriptions are important to users when deciding if they want to listen to a given episode or not. These descriptions often mention the participants of the episode and the topic of discussion. However, podcast creators frequently use episodes descriptions to promote social media links or advertisements. We call such promotional content as "boilerplate" and automatically detecting such content has been already studied in \cite{reddy2021detecting}. This is an important task because we do not want our models to mimic this behavior of generating boilerplate which would most likely end up in hallucinating URLs or social media handles. Therefore, we have decided to remove boilerplate from episode descriptions as a pre-processing step. However, no dataset for podcast boilerplate was available in Portuguese, so we created it by manually annotating a random sample of 1000 episode descriptions.
In order to increase variability in the descriptions, we also filtered out the top 5 most common repeated descriptions. For example, the Horoscope show releases episodes on a daily basis but always uses the same description "Ouça o episódio de hoje para saber tudo sobre o seu dia...".

We used the tool doccano\footnote{https://github.com/doccano/doccano} to annotate the sentences containing boilerplate. We considered any of the following as boilerplate:

\begin{itemize}
\item Contact information such as "Send in voice message http://anchor.com/foobar"
\item Social media promotion
\item Advertisements
\item Technical staff information such as producer, editor, sound technician.
\item Hashtags to characterize or promote the content
\item Credits to the soundtrack used during the episode
\item Time marks such as "0:30 <topic 1> 1:25 <topic 2> 5:40 <topic 3>"
\item License information such as Creative Commons license
\item Social media handles such as "@ladygaga"
\end{itemize}

The final dataset was comprised of 5145 sentences where 1404 were boilerplate sentences and 3741 were not. In table \ref{tab:boilerplate-examples}, we list a few examples of sentences annotated as boilerplate.

This dataset was later used to remove boilerplate from episode descriptions by training a binary sentence classifier which detects such content. In the next section, we will go into more details about the boilerplate detection method.

\begin{table}[h]
\centering
\begin{tabular}{p{0.8\linewidth}}
\hline
\textbf{Boilerplate examples}                                                                   \\ \hline
Não deixe de nos seguir nas redes sociais através do @aceleraecarreira no Instagram e Facebook. \\ \hline
Para saber mais sobre o Projeto DEFCOM, acesse: \_\_LINK\_\_                                    \\ \hline
O Toni esta no instigaram (@toni\_\_vicente) e podem encontrar o canal dele \_\_LINK\_\_ | Falem connosco e deixem as vossas sugestões no twitter @techuntalked \\ \hline
Send in a voice message: \_\_LINK\_\_                                                           \\ \hline
Linkedin: \_\_LINK\_\_    Instagram: \_\_LINK\_\_    Canal no Telegram: t.me/productgurus       \\ \hline
Ju \& Ric - Divagando Pelo Mundo: \_\_LINK\_\_/divagandopelomundo *** Novas regras para visitar o Camboja: *** Mande um recado para o Viajão! \_\_              \\ \hline
\end{tabular}
\caption{Examples of sentences annotated as boilerplate in Portuguese.}
\label{tab:boilerplate-examples}
\end{table}

\subsection*{Data preparation}

Cleaning ads, boilerplate


\subsection*{Methodology}
baselines
longformer
finetuning monolingual

\subsection*{Results and Discussion}


==> archive/sections/5_classification.tex <==
\section{Genre Prediction: Classification task}

Podcasts have become an important medium for entertainment and information dissemination. Podcast genres are important to understand user taste and recommending related listening experiences. In this task we use the podcast name and description information to classify it into one of the 19 existing genres in a supervised learning task. 

\textbf{TODO - get more information from the report document here - $https://docs.google.com/document/d/12yXKpvOBL3fP6F4wbk3cM7xlXdOkt1dbS_WsLEY1WdE/edit?usp=sharing$
}

\textbf{code: $https://ghe.spotify.net/nlpresearch/pt-dataset-classification-baseline$ }

Brief approach:
\begin{itemize}
    \item Preprocessing: 80:20 split for train test. Making sure that the show-uri is either in the train split or in test split. This condition is to avoid any information leakage between test and train splits. 
    \item Feature processing: The episode-name and episode-description is processed using 'bert-base-multilingual-uncased' resulting in a 768 size embedding for each feature. 
    \item classification: the code repo consists of the code for the 3 experiment configurations. Genre prediction using episode\_name\_embeddings, episode\_description\_embeddings, and concatenation of the two. 
\end{itemize}

Main conclusions - Description adds to the accuracy of the genre prediction task. We are also surprised to see that just the name information is also very good at predicting the genre information. Combining both description and name information for genre prediction yields the best results so far. 

==> sections/0.5_abstractwithoutresults.tex <==
\begin{abstract}
In this paper we describe the Portuguese-language podcast dataset we  have released for academic research purposes. We give an overview of how the data was sampled,  descriptive statistics over the collection, as well as  information about the distribution over Brazilian and Portuguese dialects.
We give results from experiments on \textit{a case study} showing that \textit{X}. We also show experiments on \textit{another case study}. 
Combining this collection with previously released English-language collection opens up the potential for multi-modal, multi-lingual and multi-dialect podcast information access research.
\keywords{Dataset  \and Podcast  \and Spoken audio \and Speech retrieval \and Multi-modal \and Summarization}  
\end{abstract}  
